The Future of Open Human Feedback

Human feedback on conversations with language language models (LLMs) is central to how these systems learn about the world, improve their capabilities, and are steered toward desirable and safe behaviors. However, this feedback is mostly collected by frontier AI labs and kept behind closed doors. In this work, we bring together interdisciplinary experts to assess the opportunities and challenges to realizing an open ecosystem of human feedback for AI. We first look for successful practices in peer production, open source, and citizen science communities. We then characterize the main challenges for open human feedback. For each, we survey current approaches and offer recommendations. We end by envisioning the components needed to underpin a sustainable and open human feedback ecosystem. In the center of this ecosystem are mutually beneficial feedback loops, between users and specialized models, incentivizing a diverse stakeholders community of model trainers and feedback providers to support a general open feedback pool.

==> graveyard.tex <==
\yacine{Data Protection Agencies are still proposing new rules for AI training data - for example the French DPA's latest guidelines here: https://www.cnil.fr/fr/developpement-des-systemes-dia-les-recommandations-de-la-cnil-pour-respecter-le-rgpd.}

\yacine{There are two main technical issues: allowing people to remove their data from the main version of the dataset, and propagating these removals. For the first one, whenever users of a system are giving feedback while logged in, a hash of the username may be enough to enable removal - but could be subject to abuse if random people ask for mass removals of others' data. The next more complex option is to work with the system providers to give an opt-out option inside their system while logged in. BigCode does this by requiring opt-out requests to come from a logged in GitHub user. The easiest way to do this would be to give providers a key and have them send encoded username hashes.}

\yacine{As far as propagating opt-outs, asking for removals from all trained models and derived datasets is too much to ask. BigCode handles this by requesting that new model trainings and derived datasets use the latest version of The Stack, which has opt-outs enacted.}

% [WHY] Why do we bring up this topic in the paper? Why is this relevant to open human feedback?
% [WHAT] what are the challenges to get it right? What are the nuances of the issue?
% [HOW] have people already try to approach this problem. What's the pros and cons?
% [WHAT NOW] What do we still need / recommend for progress , a better or idealised future

\begin{comment}

\section{Can we work together? For what purpose?}

We see data for AI training as an avenue that can also be shared 


\sara{some of the literature review we did for the aya dataset paper may be helpful here, just sharing it below in its entirety for reference -- but could be a useful framing point for building on.}

Prior participatory research initiatives have centered around regions or specific tasks like translation, character recognition or audio segmentation and transcription. For example, \citet{Clanuwat2018DeepLF} tackle the problem of reading and understanding \textit{Kuzushiji}, a cursive style of \texttt{Japanese} writing no longer in common use. Another example of culturally diverse data collection is MaRVL (Multicultural Reasoning over Vision and Language), which recruited native speakers from five languages (\texttt{Indonesian, Swahili, Tamil, Turkish}, and \texttt{Mandarin Chinese}) that are typologically, genealogically, and geographically diverse, to provide images of concepts that are representative of their cultures \citep{liu-etal-2021-visually}. Then, they recruited native-speaking professional linguists to write captions for these images. However, this dataset is small (less than 8,000 data points) and thus limited to evaluation only. 
\citet{hernandez-mena-meza-ruiz-2022-creating} created eight freely available resources for Mexican and Latin American Spanish by setting up a social service program that enabled students to contribute voluntarily and help with data collection for tasks like audio segmentation and transcription.
It is worth noting that these works are solely focused on the image and speech domains, unlike our work, which concentrates on text.

\citet{CaneteCFP2020} led an effort to collect a Latin American Spanish dataset and train a language model. \citet{guevara-rukoz-etal-2020-crowdsourcing} present a study focusing on the creation of a crowd-sourced corpus for Latin American Spanish dialects to address the scarcity of resources for these languages. \citet{forall-nekoto-etal-2020-participatory} focus on the task of Machine Translation (MT), and curate a dataset in 30 under-represented African languages according to a participatory research framework. \citet{cahyawijaya2023nusacrowd} focus on collection and unification of available data sources for Indonesian languages via the NusaCrowd initiative. The ongoing SEACrowd \footnote{\url{https://github.com/SEACrowd}} initiative is a similar effort focused on standardization of data resources for all South-East Asian languages. \citet{singh2024aya} created the most extensive multilingual collection to date, comprising 513 million instances through templating and translating existing datasets across 114 languages.

Many of the efforts described above describe participatory research projects with the goal of a static research release, rather than an evolving dataset which changes over time.


Why
General how
\subsection{Could a solution exist} 
Discussion of solutions to similar problems

% Soumith take a look?
In many technological areas there is a strive to find the best method, one that optimizes a metric. However, in social behavior it is much harder to define such a metric well. Because of that, it is much harder to predict what method would work the best. Moreover, it is often a strength of large communities that no single method dominates, while standards may occur \citep{}, the diversity allows for covering more usecases and for evolving methods over time.

In this spirit, we do not offer a single approach that would dominate every other effort. Instead, we consider a myriad of approaches and highlight problems that require thought and encourage us and the community to tackle them in multiple ways at once, in a way that benefits from the multiple contributors but also does not force a centralized planning of how to gather data and annotations.


\subsection{What data: Data Sources and Acquisition}
Human-model and models interact in several places,
at the time of writing this paper. They may run them locally on their own hardware \citep{}, they may use some service that as part of it includes a chatbot \citep{} and there are UIs that allow communication with models, some of which are community built \citep{hfchat,spaces}.
Depending on the above, the best way to share such conversations may differ.

One way to acquire data is that users would share their own chats. This was previously done by shareGPT \citep{} that allowed users to copy and paste chats from the proprietary chatGPT UI \citep{}, but this has siezed sharing data. A more recent effort is a plug-in \citep{} that allows users to opt-in to automatically share their chats into a larger pool of chats, shareLM \citep{}.

It is possible users would also create chats for the purpose of sharing at dedicated platforms, a survey or a form. While that is less sustainable (\S\ref{sec:sustain}) it might be beneficial for dedicated purposes such as specialized models (\S\ref{sec:}).

Another option for sharing is from the creators of the UIs. Under the right conditions (see \S\ref{sec:privacy}), the UI owners, service maintainers and space creators can choose to contribute the communications on their service. 
System-provided logs: anonymized conversation logs automatically shared by AI systems. 

Another source that may enable sharing if not share directly is the platforms allowing the UI. For example, Hugging Face hosts about 1K assistants \citep{}, and most spaces use chatUI \citep{} or GradIO \citep{} to create chats. Due to that, if a platform makes sharing accessible it will instantly allow many to share with substantially less effort.

Discuss the trade-offs between different data sources in terms of value, privacy, and user agency. 

Propose strategies for obtaining informed consent and managing data ownership rights in a transparent and ethical manner.

\subsection{What Annotation: Annotation Sources and Types}
[\mimansa{Draft allocation 13 March}]
Compare and contrast the value of annotations from different sources: 

Interaction annotations: insights from the user directly interacting with the AI model. 

Interlocutor annotations: insights from the user directly giving feedback for the AI model. 

Third-party annotations: observations and feedback from external specific annotators. 

Expert annotations: specialized knowledge and insights from domain experts. 

Discuss the potential for enabling novel annotation approaches and methodological innovations within an open framework. 

Explore strategies for integrating and reconciling annotations from multiple sources to enhance data robustness and reliability.

\subsection{Quality Assurance and Consensus-Building}
[\mimansa{Draft allocation 13 March}]
Discuss the importance of maintaining data quality and address the challenges of identifying and addressing: 

Low-quality annotations due to lack of expertise or attention. 

Biased annotations reflecting individual or societal biases. 

Malicious annotations intentionally introduced to harm the system. 

Propose mechanisms for: 

Data validation and filtering techniques 

Community moderation and peer review processes 

Algorithmic approaches for anomaly detection and bias mitigation 

Explore strategies for resolving disagreements among annotators, including: 

Voting mechanisms 

Discussion forums and collaborative decision-making 

Expert adjudication for complex or contentious cases 

Discuss the importance of developing community guidelines and moderation processes to ensure a safe, inclusive, and productive annotation environment.

\subsection{Categorization and Structure}
[\mimansa{Draft allocation 13 March}]
Discuss the importance of organizing annotations by task, domain, style, and complexity to enable: 

Targeted model training and evaluation 

Comparative analysis across different contexts and applications 

Efficient retrieval and utilization of relevant feedback data 

Propose the development of standardized taxonomies and ontologies for annotation to ensure consistency, interoperability, and facilitate knowledge sharing.

\end{comment}



\begin{comment}
    
\thc{some relevant examples from a prior project..
Cornell eBird, Ushahidi, openstreetmap, wikipedia
}
\thc{we may also want to consider including collaborative QA platforms like StackExchange, askubuntu, quora as examples of (non-data centric) peer production projects that are relevant.}

Note for this section:

Social media flagging: Highlight how users contribute to content moderation. (like community notes)

Identify factors contributing to the success of these projects: 
\thc{we should read fairly close into the peer production literature, e.g. hills' works https://mako.cc/academic/hill-almost\_wikipedia-DRAFT.pdf, https://mako.cc/academic/benkler\_shaw\_hill-peer\_production\_ci.pdf, https://wikipedia20.mitpress.mit.edu/pub/lifecycles/release/2
 as well as the OSM contributor survey https://journals-sagepub-com.stanford.idm.oclc.org/doi/epub/10.1177/0002764212469364
}

Gamification and motivation: Explore how rewards, recognition, and gamification elements can incentivize participation and sustained contributions. 

Community and reputation: Discuss the role of community building, shared purpose, and reputation systems in fostering trust and ensuring data quality. 

\thc{shared purpose / the mission + user perception on the achievability of that mission seems to factor in heavily in many of the peer production community surveys I've read.}

Extract lessons learned from these projects and discuss their applicability to AI development and open human feedback systems.

\thc{note also that there's a large literature on innovation contests that may also be relevant and enable distributed contributions to the whole. efforts like datacomp go down this vision and may be worth noting.}

Wikipedia: Discuss its collaborative content 
\thc{wiki's moderation mechanisms are also very interesting given its very inclusive goals. e.g. mission statements that clearly outline what is in and out of scope  https://en.wikipedia.org/wiki/Wikipedia:What\_Wikipedia\_is\_not}

creation and maintenance model. 

OpenStreetMap: Analyze its community-driven approach to geospatial data and services. 

\end{comment}

\begin{comment}
\section{Risks, Challenges, and Ethical Considerations}
\subsection{Privacy and Security Risks}
Discuss potential privacy and security risks associated with collecting and sharing user data in open human feedback systems, including: 

Data breaches and unauthorized access 

Re-identification of anonymized data 

Misuse of personal information for malicious purposes 

Propose mitigation strategies: 

Implementing advanced security measures and privacy-preserving techniques, such as differential privacy and federated learning. 

Developing incident response plans and data breach notification protocols. 

Establishing clear accountability mechanisms and data governance structures.

\subsection{Bias and Fairness Concerns}
Address the risk of perpetuating existing biases and introducing new biases through user-generated data in open annotation systems. 

Discuss the need for: 

Diverse representation of annotators to mitigate individual biases. 

Algorithmic fairness and transparency in model development and data collection processes. 

Implementing bias detection and mitigation techniques.

\subsection{Exploitation and Fair Compensation}
Discuss the ethical considerations of engaging volunteer annotators and the potential for exploitation. 

Explore ways to ensure fair compensation and recognition for contributors, including: 

Monetary rewards and micro-payments 

Public acknowledgement and community recognition 

Attribution and intellectual property rights considerations 

Advocate for developing ethical guidelines and best practices for human-in-the-loop AI systems that prioritize the well-being and fair treatment of annotators.

\subsection{Addressing the Capabilities Gap}
Discuss the challenges of human evaluation and inclusion of increasingly advanced and complex AI systems in annotation (RLAIF). 

Propose strategies for bridging the capabilities gap between human annotators and AI models: 

Providing education, training, and specialized tools for annotators to enhance their understanding and evaluation skills in terms of evaluating an LM answer. 

Fostering collaboration between AI experts and domain specialists to leverage their combined knowledge and expertise.

\subsection{Societal Impact and Responsible AI Development}
Discuss the potential consequences of AI systems trained on open human feedback, both positive and negative. 

Emphasize the need for ongoing monitoring, auditing, and adjustment of models to ensure they remain aligned with human values and societal expectations. 

Advocate for engaging diverse stakeholders in the development and governance process of AI systems to ensure responsible and inclusive AI development.
\end{comment}


% Distributed computing and data management infrastructure 
% Efficient annotation workflows and task allocation 
% Leveraging AI-assisted tools for annotation support and efficiency, such as pre-annotation, suggestion mechanisms, and quality control algorithms 
% Discuss the importance of designing user-friendly interfaces and intuitive annotation tools to facilitate participation and ensure data quality.
% Discuss the challenges of scaling open human feedback systems to accommodate large-scale AI development and vast amounts of data. 

\begin{comment}
\subsubsection{The Historical Role of Volunteer and Crowd Labor in Technology}
\textcolor{red}{HRK to start this section}

\subsubsection{Participatory and Inclusive}
Emphasize the importance of engaging a diverse community of contributors to ensure data representativeness and inclusivity, addressing historical biases and underrepresentation. 
\textcolor{red}{HRK to start this section}


\subsubsection{Motivating Participation}
Explore various incentive mechanisms to encourage high-quality and sustained user contributions: 

Gamification elements: points, badges, leaderboards, challenges. 

Rewards and recognition: financial incentives, public acknowledgement, community reputation. 

Intrinsic motivation: fostering a sense of purpose, belonging, and contributing to AI advancement. 

Discuss ethical considerations and the importance of avoiding exploitation of annotators, ensuring fair compensation and recognition for their contributions.

\end{comment}
\begin{comment}

Incentives are key to sustainable and continuous participation
Highlight the need for ongoing data collection and feedback to capture evolving user behaviors, preferences, and societal norms. 

Discuss strategies for integrating data collection and annotation into everyday AI model use, making the process seamless and sustainable. 

Explore incentive structures and motivational mechanisms to encourage long-term participant engagement, including: 

Gamification elements and rewards 

Recognition and appreciation for contributions 

Community building and fostering a sense of ownership

\thc{I think maybe even more than the above, a clear mission statement is really important e.g. ``make encyclopedic knowledge available to everyone'' or ``map information should be free''. I think having a clear mission statement that participants think is achievable is pretty critical to the success of things like this.}

\thc{Also, do we want to bring up community management? it's quite hard and there's some tricky stuff like https://wikipedia20.mitpress.mit.edu/pub/lifecycles/release/2
which makes it very hard to sustain a strong peer production community for a long time.}

\end{comment}

\subsection{Scaling Human Preferences with Infrastructure}

% [WHY] Why do we bring up this topic in the paper? Why is this relevant to open human feedback?
The collection of human preference data is dependent on personal labour attributes like an individual's remuneration, qualification, motivation, or precariaty.
Therefore, the implementation and scaling of human feedback projects has a relationship with both the subjects' quality of life and the collected data's quality and value. 
Scalable infrastructure mobilises larger teams to supply preferences, which in turn facilitates higher quality data at larger scales. 
Pre-annotating large collections of data with language models reduces manual work and isolate humans to the most skilled and/ or interesting tasks.
Until recently, examples of automated preference collection were restricted to private industrial scale projects.

% [WHAT] what are the challenges to get it right? What are the nuances of the issue?
Synthetic preference collection using language models reduces labour impact on individuals.
Synthetically labelled datasets have lead to the successful language models on benchmarks \citep{llama3}. \cite{phi3} filtered and improved existing datasets using generative language model to create a high quality subset of data for training \citep{ultrafeedback, phi3}.
Distilling datasets using existing generative models presents a fundamental challenge. 
The fixed body of knowledge that the dataset begins with is reduced down to higher quality abstractions, without new information \citep{shumailov2024curse}.
Without broadening and diversifying the knowledge base, a dataset's representation of the world is limited.

% [HOW] have people already try to approach this problem. What's the pros and cons?
FineWeb
WizardLM
UltraFeedback

% [WHAT NOW] What do we still need / recommend for progress , a better or idealised future.
Projects like FineWeb show that community initiatives can offer open datasets improved by synthetic feedback.
However, such projects still require expensive compute infrastructure that is not accessible to all communities.
Future work should target both open and free resources to mobilise domain specific minority groups to scale preference projects with synthetic feedback (c.f., \ref{adaptable-and-up-to-date}).




\section{Open Questions and Future Directions}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Conclusions
% 200 words
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Interaction as Implicit Annotation}
% \textcolor{red}{[HRK]} I feel like this could go in a section about \textbf{Methodology} or how we collect human feedback in the main body of the paper.



% \textcolor{blue}{[Shachar Don-Yehiya]}
% So far we have discussed efforts to annotate data, during the human-model interaction or in retrospect. Another direction to consider is leveraging implicit cues in the human-model interaction \citep{hancock-etal-2019-learning}, to automatically extract feedback. Such naturally occurring feedback can be in the form of free text, with the user directly referring to the quality of the model's response (e.g. 'thank you!', or 'that's wrong'), or more implicit, for example, the user moves to ask their next question, usually only after they are satisfied with the previous answer.

% This approach has two notable advantages. First, this feedback is freely given, without human annotation effort. Second, this form of feedback is potentially closer to the feedback given by two human interlocutors, possibly containing relevant information for better alignment.

% Implementing techniques to infer implicit feedback will require data   


% Explore the potential for leveraging user behavior and engagement patterns with AI systems as implicit feedback. 

% Discuss the benefits and challenges of using implicit signals alongside explicit annotations. 

% Propose research directions for developing techniques to infer and validate implicit feedback accurately and ethically.

%\subsection{Personalization and Adaptive Feedback Loops}
%Discuss the opportunities for creating personalized AI experiences through individual-level feedback and adaptive learning algorithms. 

%Explore how open human feedback can facilitate continuous refinement of models based on user interaction and real-time feedback. 

%Address the ethical implications of personalization and ensure user control over the data and algorithms used to tailor their experiences.

\subsection{Scaling Human Input for Advanced AI Systems}
Discuss the challenges of scaling human input and feedback mechanisms to accommodate increasingly capable and autonomous AI systems. 

Explore potential solutions: 

Developing hybrid human-AI annotation approaches that leverage the strengths of both humans and machines. 

Fostering collaborative intelligence where humans and AI systems work together to solve complex problems and provide feedback. 

Ensuring human oversight and alignment remain central to AI development, even as models become more advanced.

\subsection{Domain-Specific Considerations}
[\mimansa{Draft allocation 13 March}]
Acknowledge the unique challenges and requirements for open human feedback across different application domains (e.g., healthcare, finance, education). 

Discuss the need for developing: 

Specialized annotation frameworks and guidelines tailored to specific domains. 

Quality metrics and evaluation methods relevant to each domain. 

Collaboration with domain experts and stakeholders to ensure the feedback system meets the specific needs and challenges of the application area.

\subsection{Long-Term Sustainability and Governance}
Discuss the importance of establishing sustainable funding models and institutional support for open annotation efforts. 

Explore potential funding sources: 

Government grants and public funding initiatives 

Industry partnerships and corporate social responsibility programs 

Crowdfunding and community-based support 

Discuss the need for developing governance structures and decision-making processes for open human feedback systems: 

Ensuring transparency and accountability in data collection, annotation, and model development processes. 

Facilitating public participation and stakeholder engagement in the governance of AI systems.

% Outreach and education initiatives 

% Accessible and user-friendly annotation tools 

% Community building and fostering a sense of shared purpose 

% Addressing language barriers and cultural differences 

% Discuss the importance of balancing representation with data quality, ensuring that contributions are accurate and reliable.

% Large Language Models are increasingly used as economical alternatives to human participants across various domains such as computational social science, user testing, annotation tasks, and opinion surveys. However, the utility of LMs in replicating human demographic nuances is limited by inherent training constraints. Notably, they often fail to accurately portray the diverse perspectives of different demographic identities due to their training on decontextualized text snippets and optimization for prevalent responses rather than accurate or representative ones. This can result in the stereotypical portrayal and oversimplification of complex human identities, known respectively as misportrayal and group flattening. Such limitations necessitate cautious application of LMs when replacing human roles that require nuanced understanding of varied human experiences .

%The effort each individual needs to contribute is a key factor in the success of distributing work and achieving participation. There are always more people agreeing to make a minimal effort than to perform more sizeable tasks. Moreover, when a part of the task is repetitive or wasteful, it wastes the time of many, unlike in centralized efforts where the overhead is limited to a small number of contributors. These issues are more relevant to annotation, as we assume most chat data would be contributions of chats that would have been made anyway.

Large Language Models (LLMs) have emerged as cost-effective alternatives to human participants in various domains, such as computational social science, economic surveys, online surveys, and focus groups~\citep{X}. However, the ability of LLMs to accurately replicate the demands of a particular human demographic is constrained by training limitations. Specifically, the data used to train LLMs and the demographics of the individuals who generated that data can lead to stereotypical portrayals of humans~\citep{X}. This raises concerns about the representativeness of LLM outputs and their alignment with the nuanced responses of specific human demographics. To address this limitation, human annotations and participation remain crucial in the development and refinement of LLMs. Rather than relying solely on LLM developers and technologically adept groups, it is imperative to obtain a more diverse perspective towards human development in LLMs. Developers are employing various methods to create more diverse LLM integrations, such as incorporating different languages, dialects, and in-group communication patterns~\citep{X}. Factors like ethnicity, gender, age, and education level, as reflected in the training data, can significantly influence the model's output~\citep{X}. To achieve greater diversity, targeted strategies should be implemented to encourage participation from diverse groups in the annotation process. This can be accomplished through outreach initiatives, targeted recruitment efforts in educational institutions, and collaborations with domain experts in hospitals and community organizations~\citep{X}. By involving a broader range of participants, LLM developers can gain a more comprehensive understanding of the model's performance across different demographics.

When aligning incentives for participation, it is crucial to consider the diverse needs and interests of different language communities and subcultures. In-group language and terminology can vary significantly across academic disciplines, professional fields, and social groups~\citep{X}. Providing accessible and user-friendly annotation tools with intuitive interfaces, multi-language support, and inclusive design can lower the barrier to entry and enable individuals from various backgrounds to contribute effectively~\citep{X}. By accommodating the linguistic and cultural differences among participants, LLM developers can ensure a more representative and inclusive annotation process.


Ensuring the quality and reliability of the collected data is essential, but it is important to acknowledge the subjectivity inherent in certain tasks, such as evaluating the quality of LLM-generated essays. Opinions on what constitutes a "good" output can vary among individuals, necessitating the gathering of diverse perspectives~\citep{X}. Establishing clear guidelines for data collection and annotation, investing in the training and support of diverse annotators, and regularly auditing the data for biases or gaps in representation can help maintain data quality while recognizing the subjective nature of certain tasks~\citep{X}.

Ultimately, the question of alignment arises: to whom or what should the LLM be aligned? Capturing the diversity of perspectives, experiences, and languages in LLM alignment is crucial to ensure that the models serve the needs and interests of a wide range of users~\citep{X}. Engaging with diverse participants and end-users, conducting extensive testing and evaluation across different contexts, and iteratively refining the model based on feedback from diverse user groups can help achieve this balance~\citep{X}. By prioritizing diversity and inclusivity in LLM development and annotation, we can create models that better represent and serve the complex tapestry of human experiences and perspectives. Future research should focus on developing robust methodologies for engaging diverse communities, evaluating the representativeness of LLM outputs, and refining alignment strategies to better serve the needs of a wide range of users.



INTRO GRAVEYARD

%%% DONT EDIT THIS SECTION IT IS OLD%%%%%%

%     \section{Introduction}
%     \hrk{Don't edit this section its, old. I'm not moving to graveyard because comments can't be copied}
%     % Ramon: any reason to use LMs and not LLMs?
%     Large language models (LLMs) such as GPT, Claude, LLaMA or Gemini are capable of answering diverse queries and conversing about countless topics. To achieve such abilities, such language models are first pre-trained on trillions of tokens of text and then fine-tuned on a much smaller set of carefully created user interactions and user feedback, improving their conversational abilities in response to specific questions or preventing unwanted behaviors.
    
%     \emph{Chats} conducted between humans and models contain invaluable information (See \S\ref{sec:motive_chats}). They can tell us what are those models really used for, what tasks are they failing, who are they serving, and how are human and machine languages affected by interactions. All those questions and many others require  data. Fortunately, given the large increase in performance in recent years,
    
%     With the right annotation for those chats the potential is larger still (See \S\ref{sec:motive_fb}). Chat annotation can allow for improving the models, creating models that serve specific tasks, analyzing errors, and preventing misinformation, among others. Those in turn open the door to better models that can be improved again in a continual cycle of aligning models to the morals and benefits of humanity.
    
%     With those obvious benefits, one may ask, why isn't it done? In fact, it is done, but mostly behind the curtains of tech companies in a way that is fundamentally closed in multiple aspects (see \S\ref{sec:closed}). The process utilized is largely is closed and little information about it is available, the data obtained is closed to public access, the organization of the annotator teams is also closed, without the possibility of voluntary participation, and finally the scope and duration is also closed with intensive annotation streaks that iteratively improve one single model.
    
%     Despite the advantages of having such open data, gathering it is not a simple feat.
%     The immense impact of LMs pushed for an alternative to closed APIs -- open-weight models. Those bring about a mixed blessing, when anyone can run a model, collecting its outputs must become a shared endeavour. This is the challenge we are facing, how to create fair, sustainable and functioning processes that combine the shifting needs, wishes, expertise and motivations of large groups. These traits pose a challenge, but also an opportunity, under the right circumstances (see \S\ref{}) massive groups can greatly split tasks or pinpoint specialists performing immense tasks with minimal effort for each individual.
    
%     We ourselves keep true to those challenges and advantages, this paper is the outcome of a collective effort of *** experts in topics such as LM training, open source, data, annotation, legal, human experimentalists, reinforcement learning and other aspects, gaining from the diverse expertise and abilities of the group.
    
%     %purpose and structure of the paper
%     This paper highlights the need for a sustainable way to gather chats and annotations over chats in open endeavors. We go further and characterize what would be needed to create the right environment allowing such efforts. Last, we propose our vision to tackle the different goals and challenges to make our common dream a reality. 
    
%     % structure of the paper
%     %Elaborate on the previous one or add here more on the structure 
%     % add especially interesting bottom lines (we proposed a decentralized XYZ, we see this as most likely to succeed through diverse aproaches at once etc.)
    
    
%     \subsection{Language Model training and alignment phases}
    
%     Although there are other types of AI models (e.g. vision models, multimodality), in this paper we focus on Language Models (LMs). 
%     Language models are built from a large collection of numerical parameters that represent language and typically number in the billions. Model artifacts are referred to as \emph{weights} which are optimised through a \emph{training} process on samples of data.
%     The development of LMs encompasses two phases: pretraining and alignment, each critical to the model's functionality and application efficacy.
    
%     % define LM pretraining
    
%     During the initial pretraining stage, LMs are exposed to extensive corpora of textual data in an unsupervised learning format. The core activity involves predicting subsequent words from given contexts without direct human oversight \citep{narayanan2021, yangxlnet}. Although this phase operates without direct annotation, strategic curation of input data is employed to enhance the quality and relevance of the training material \citep{bigscience-2022-bigscience, rae2022scaling}. This phase is fundamental as it builds the model's preliminary understanding of language, laying the groundwork for advanced processing capabilities. However, it stops short of preparing the model for conversational engagement or complex task execution.
    
%     \thc{probably worth acknowledging the increasing trend of mixing the SFT data into the tail end of pertaining (two phase training). this makes it a bit harder to modularize alignment as its own component.}
    
%     % define LM alignment phase
%     Following pretraining, LMs undergo an alignment phase that is instrumental in refining their output to align with human expectations and preferences \citep{wang2023aligning, guo2024humaninstructionfree, tunstall2023zephyr}. 
%     Alignment uses transfer learning method to fine-tune the base model toward human expectations of instruction.
%     %This phase leverages supervised learning and reinforcement learning to fine-tune language models based on human input. 
%     During alignment, various forms of feedback are utilized; participants may select preferable responses from multiple options, provide positive examples, or rate answers to guide the model’s learning trajectory. This stage is crucial for enhancing the model's ability to follow instructions and engage in coherent dialogue \citep{}.
    
%     % END Paragraph defining AI and types of AI
    
%     \subsection{The importance of chats for LMs} \label{sec:motive_chats}
    
%     The alignment phase uses chat data to expose models to the preferences of humans, guiding them in generating responses that are not only accurate but also more ethical, safe, and contextually appropriate. Without alignment, models might interpret a command in a way that is technically correct but ethically questionable, dangerous, or unhelpful. 
    
%     \textbf{TODO: explain more on efforts to collect chats (feedback is next section) and motivate why we need it, and why what exists is not enough (e.g., models change)}
    
%     Community efforts to build alignment datasets comparable to \citet{bai2022training} have utilized the browser extension  \citep{ShareLMS76:online} to integrate data from chat applications with shared datasets. 
    
%     \thc{what about open assistant? seems like the somewhat clear prior attempt in this space}
    
    
%     \subsection{Forms of Human Feedback }
%     % BEGIN Paragraph defining human feedback
%     Human feedback refers to the process where human annotators provide evaluations or corrections to machine-generated outputs, such as texts produced by natural language processing (NLP) models. This feedback is crucial for refining and training machine learning models, particularly in tasks involving natural language understanding and generation. The goal of integrating human feedback is to harness human insights to enhance the machine's learning process, ensuring that the models developed are not only more accurate but also helpful and follow instructions. Human feedback in this framework typically involves several key components:
    
%     Annotation: Human annotators review the outputs produced by a model and provide labels or corrections. For example, in a text classification task, annotators might label text according to sentiment or topic categories. In translation or summarization tasks, they might correct errors or suggest improvements.
    
%     Assessment: Annotators assess the quality and accuracy of machine-generated text against predefined criteria, which can include helpfulness, relevance to a prompt, or fidelity to a source text in translation tasks.
    
%     Guided Correction: Feedback often involves not just identifying errors or misclassifications but also guiding the model towards correct outputs. This might be done through direct edits to the text or by providing more structured feedback, such as rules or examples.
    
%     Iterative Refinement: Human feedback is usually part of an iterative process where the model is continually updated based on the latest feedback. This iterative loop helps the model to gradually improve its accuracy and reliability.
%     % END Paragraph defining human feedback
    
%     \subsection{Role of Human Feedback in the Machine Learning lifecyle}
%     Explain the various roles of human feedback throughout the AI/ML lifecycle, including: 
%     \begin{enumerate}
%         \item Training data generation and labeling 
%         \item Model evaluation and performance assessment 
%         \item Bias detection and mitigation 
%         \item Alignment with human values and ethical considerations 
%     \end{enumerate}
    
    
%     Discuss the renewed interest in human feedback due to the rise of post-training alignment techniques like RLHF. 
    
%     Emphasize the ethical implications of integrating human values and perspectives into AI systems, ensuring responsible development and deployment.
    
    
%     the concentration of economic power threatens the free market. \citet{hayek1976road} noted that competition, capitalism and the free market are important components in preventing centralized planning. Centralized planning is defined as the state taking active control over the economy, such as in Fascism or Communism. If economic competition is eliminated for some reason, such as through monopolies, this eventually leads to centralized planning, which is "inherently undemocratic".
    
%     \andi{I see a somewhat increasing gap between focus on understanding how to using use to train better models vs. understanding how humans even want to/can benefit from models. The former is a pure learning question while the latter is an interaction/social benefit question. May be worth touching on the intersection of these two.}
    
%     \subsection{Limitations of Current Closed Data Collection and Annotation Methods} \label{sec:closed}
    
%     % \textbf{TODO: explain why the current “closed” human feedback is bad. define what we mean by "closed" human feedback}
%     For-profit companies have led the creation of human feedback data in a way that is fundamentally \textit{closed} in multiple dimensions. First of all, the whole process happens behind closed doors and little details have emerged about fundamental parameters such as dataset size and content. There are some exceptions such as early works at Google i.e. LaMDA~\citep{thoppilan2022lamda}, early work related to current Claude models~\citep{bai2022training} and ChatGPT models i.e. InstructGPT \citep{ouyang2022training} as well as Meta\'s LLaMa-2 model \citep{touvron2023llama}. However, technical reports have become poorer in information in later model versions\footnotemark\footnotetext{As of date, the report for LLaMa-3 is not published which could change this trend.}. The data produced itself is with very minor exceptions closed-access and remains unknown to the public. Notable exception being AnthropicHH~\citep{bai2022training,ganguli2022red}\footnotemark\footnotetext{\url{https://github.com/anthropics/hh-rlhf}}. Annotator teams are formed, as far as we know, through contracting a selected group of professionals. This process is thus closed to voluntary participation through open crowdsourcing platforms or less controlled crowdsourcing paid work. Number of workers is also reportedly small e.g. InstructGPT, reports $40$ annotators, although this numbers is likely to be much higher for the production models. AnthropicHH is again the exception mixing $15$ workers hired through Upwork with a larger group of Mechanical Turk crowd workers \cite[App. D.1]{bai2022training}. Finally, the execution of data gathering is also closed in time and scope. As per published information, annotation efforts consist fundamentally of gathering demonstrations and feedback labels. The former correspond to complete examples of desired behaviour covering a large set of target scenarios, and the latter rankings or binary selections for a specific model. Gathering of feedback is also done for a single model and iteratively. This iterative character seems to be key, with the annotator team annotating the outputs of a model and that feedback going into the next model training through the use of a reward model, after which the process is repeated. This is a process requires high bandwidth communication between model training and annotation teams and is fundamentally closed in time.
    
%     One can take the fully closed processed above as points on an extreme of the closed-open space for which examples exist that open some of these categories. The Databricks Dolly 15k Dataset~\citep{DatabricksBlog2023DollyV2}, for example, was created behind closed doors, with annotators being limited to company employees and a set of annotation guidelines inspired by InstructGPT, but otherwise unrestricted and incentivize by an employee rewards. The gathering of data was thus closed in time and scope, but the data was fortunately made public with an non restricting license \footnotemark\footnotetext{\url{https://github.com/databrickslabs/dolly}}. Databricks Dolly 15k includes only demonstrations and no model feedback. Also, in the space of semi-open approaches ChatbotArena~\citep{chiang2024chatbot} is worth mentioning due to its relevance as an evaluation tool. ChatbotArena is a platform that collects mainly model feedback, in the form of preference ranking of the output of two models given an unrestricted annotator prompt. There is no restriction in who can join and models are sampled from an open list that evolves over time. The data has been partially released\footnotemark\footnotetext{\url{https://huggingface.co/datasets/lmsys/chatbot_arena_conversations}} along with feedback for answers to the mt-bench evaluation benchmark~\citep{zheng2023judging}\footnotemark\footnotetext{\url{https://huggingface.co/datasets/lmsys/mt_bench_human_judgments}} although the total dataset accumulated is far larger and is reportedly not released due to licensing concerns, since it uses proprietary model outputs.
%     % also https://www.interconnects.ai/p/llama-2-from-meta?sd=pf
%     Open Assistant~\citep{kopf2024openassistant} is a good example of full open approach, with full transparency in the process, open participation through a crowdsourcing platform, which implies big challenges in terms of community moderation of close around $13000$ volunteers \cite[Sec.~3]{kopf2024openassistant}. The dataset contains both demonstrations and feedback and with a large majority of demonstrations being human made, with roughly only a $5\%$ of model generated turns in total \cite[Sec.~4]{kopf2024openassistant}. This also means that the amount of model feedback is therefore limited.
    
    
    
%     While open data collection lags behind, large tech companies control vast amounts of user data. Companies collect user-model chats through their closed APIs, and spend a lot of money to annotate them using in-house annotators and annotation tools. This creates data and annotation moats, that limit access for researchers and smaller companies. In this paper, we refer to this data source as "closed" human feedback.
    
%     In addition to the accessibility problem, closed human feedback resources also suffer from scalability and diversity problems. Continue...
%     % Data and annotation moats: 
    
%     % Discuss how large tech companies control vast amounts of user data, creating data moats that limit access for researchers and smaller companies. 
    
%     % Explain the high costs and limited accessibility of annotation resources, hindering scalability and diversity in AI development. 
    
%     Lack of diversity and representation in datasets: 
    
    
%     Highlight how current datasets often underrepresent various demographics, geographies, and perspectives, leading to biased and unfair AI systems. \sara{we have an extensive literature review in aya motivating this -- also meaningful to pull charts from ai index report which characterizes contributors to research and shows massive geo divide as well as data provenance initiative paper which shows most datasets arise from western creators.}
    
%     \thc{In general, i find the Wikipedia analogy to be compelling as an argument for open vs closed in that you can get something that is just better than a closed product (encyclopedia brittanica) through the focused effort of many domain experts who each contribute}
    
%     Discuss the importance of capturing the full spectrum of human experiences and ensuring inclusivity in data collection. 
    
%     Static datasets and limited adaptability: 
    
%     Explain the limitations of static datasets in capturing evolving language, user behavior, and societal norms. 
    
%     Discuss the need for models to continuously learn and adapt to changing contexts and user needs.
    
%     \subsection{The Potential of Open Human Feedback}
    
%     \textbf{TODO: present the key argumeent of this paper: explain why "open" human feedback is needed. define what we mean by "open" human feedback}
%     \thc{there's a complexity here in thinking about moderation - much like wiki (and communitynotes, below) we will likely have to only work on topics that are consensus, objective ones.}
    
%     \wenting{https://communitynotes.x.com/guide/en/about/introduction Twitter has successfully done some community-based annotations on flagging unsafe contents. Their incentive models are interesting. This can be paid to use.}
    
%     Introduce the concept of open human feedback as a potential solution to the limitations of current data collection and annotation practices. 
    
%     Discuss how open human feedback can: 
    
%     Address data and annotation moats by democratizing data collection and enabling wider participation. 
    
%     Promote diversity and representation in datasets by engaging a broader range of contributors. 
%     \thc{Probably also worth noting (maybe later for challenges with open data?) that it's hard to get diverse representation in peer production efforts as well. We can point to Wikipedia contributor distributions, this (https://journals-sagepub-com.stanford.idm.oclc.org/doi/epub/10.1177/0002764212469364) survey on openstreetmap, etc.}
    
%     Enable continuous learning and adaptation of models through ongoing feedback loops. 
    
%     Support a wider range of AI research and applications by providing access to diverse data and perspectives.
    
%     \subsection{Purpose and Structure of the Paper}
%     State the paper's objectives: 
    
%     Advocating for the adoption of open annotation systems in AI development. 
    
%     Proposing frameworks and guidelines for integrating open human feedback effectively and ethically. 
    
%     Briefly outline the research methodology employed in the paper, including literature review, case studies, and theoretical analysis. 
    
%     Provide a roadmap of the paper's sections and main arguments, guiding the reader through the content and structure.
    
%     % \section{Background and Literature Review}
%     % make sure all is integrated somewhere
    
%     % \subsection{The Role of Data and Annotation in Machine Learning}
%     % Provide a primer on data annotation in AI/ML: 
    
%     % Define different types of annotations (e.g., classification, labeling, rating, bounding boxes) and their purposes. 
    
%     % Discuss how annotation impacts various stages of the AI/ML lifecycle, from training and evaluation to deployment and ongoing refinement. 
    
%     % Explore different categories of human feedback: 
    
%     % By involvement level: casual user feedback vs. expert evaluation. 
    
%     % By quality demands: low-effort ratings vs. high-effort, detailed annotations. 
    
%     % By feedback modality: explicit (e.g., ratings, comments) vs. implicit (e.g., user interactions). 
    
%     % Discuss considerations for pre-training and post-training data: 
    
%     % Highlight the potential of open human data in both pre-training and post-training phases. 
    
%     % Discuss the current emphasis on post-training human feedback and the need for more diverse and dynamic pre-training data.
    
%     % \subsection{Current Landscape of Data and Annotation Efforts}
%     % Survey existing efforts and platforms for AI data collection and annotation, including commercial and academic projects: 
    
%     % Examples: Amazon Mechanical Turk, Prolific, Dynabench
    
%     % Analyze the strengths and limitations of these approaches, considering factors like: 
    
%     % Data access and sharing policies 
    
%     % Diversity and representativeness of annotators 
    
%     % Quality control mechanisms 
    
%     % Ethical considerations and potential for exploitation 
    
%     % Identify best practices and innovative approaches that can inform the design of open human feedback systems.


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

